Observation and Spectral Measurements of the Crab Nebula with Milagro

The Crab Nebula was detected with the Milagro experiment at a statistical significance of 17 standard deviations over the lifetime of the experiment. The experiment was sensitive to approximately 100 GeV - 100 TeV gamma ray air showers by observing the particle footprint reaching the ground. The fraction of detectors recording signals from photons at the ground is a suitable proxy for the energy of the primary particle and has been used to measure the photon energy spectrum of the Crab Nebula between ~1 and ~100 TeV. The TeV emission is believed to be caused by inverse-Compton up-scattering scattering of ambient photons by an energetic electron population. The location of a TeV steepening or cutoff in the energy spectrum reveals important details about the underlying electron population. We describe the experiment and the technique for distinguishing gamma-ray events from the much more-abundant hadronic events. We describe the calculation of the significance of the excess from the Crab and how the energy spectrum is fit. The fit is consistent with values measured by IACTs between 1 and 20 TeV. Fixing the spectral index to values that have been measured below 1 TeV by IACT experiments (2.4 to 2.6), the fit to the Milagro data suggests that Crab exhibits a spectral steepening or cutoff between about 20 to 40 TeV.

==> ch.systematics.tex <==
\section{Systematic Studies}

\begin{figure}
\includegraphics[width=100mm]{figures/crab-stability.eps}
\caption{\label{crabstability}
Showing stability of the Crab
}
\end{figure}


\begin{figure}
\includegraphics[width=100mm]{figures/residuals.eps}
\caption{\label{crabstabilityResiduals }
Residuals of Crab Stability
}
\end{figure}

